OrionBench: Benchmarking Time Series Generative Models in the Service of the End-User

Time series anomaly detection is a vital task in many domains, including patient monitoring in healthcare, forecasting in finance, and predictive maintenance in energy industries. This has led to a proliferation of anomaly detection methods, including deep learning-based methods. Benchmarks are essential for comparing the performances of these models as they emerge, in a fair, rigorous, and reproducible approach. Although several benchmarks for comparing models have been proposed, these usually rely on a one-time execution over a limited set of datasets, with comparisons restricted to a few models. We propose OrionBench: an end-user centric, continuously maintained benchmarking framework for unsupervised time series anomaly detection models. Our framework provides universal abstractions to represent models, hyperparameter standardization, extensibility to add new pipelines and datasets, pipeline verification, and frequent releases with published updates of the benchmark. We demonstrate how to use OrionBench, and the performance of pipelines across 17 releases published over the course of four years. We also walk through two real scenarios we experienced with OrionBench that highlight the importance of continuous benchmarking for unsupervised time series anomaly detection.

==> tables/bench_frameworks.tex <==
% \resizebox{\linewidth}{!}{%
\small
\begin{tabular}{rrc}
    \toprule
                                                                &   \multicolumn{2}{c}{Published Leaderboard} \\
    \cmidrule(lr){2-3}
    \textbf{Benchmark Framework}                                &   Last Updated    & Source  \\
    \midrule
    \texttt{Numenta}~\cite{lavin2015numentabenchmark}     &   Jun 2018        & Github \\
    \texttt{TSB UAD}~\cite{paparrizos2022tsb-uad}         &   Nov 2022        & Github \\
    \texttt{TODS}~\cite{lai2021todsbenchmark}             &   Dec 2021        & Paper \\
    \texttt{TimeEval}~\cite{wenig2022timeeval}            &   Aug 2022        & Paper \\
    \texttt{Exathlon}~\cite{jacob2020exathlon}            &   Sep 2021        & Paper \\
    \texttt{Merlion}~\cite{bhatnagar2021merlion}          &   Sep 2021        & Paper \\
    \midrule
    \bench                                                &   Oct 2023        & Github \\
    \bottomrule
\end{tabular}

% \resizebox{\linewidth}{!}{%
% \begin{tabular}{rrc}
%     \toprule
%                                                                 &   \multicolumn{2}{c}{Published Leaderboard} \\
%     \cmidrule(lr){2-3}
%     \textbf{Benchmark Framework}                                &   Last Updated    & Source  \\
%     \midrule
%     \texttt{Numenta, 2015}~\cite{lavin2015numentabenchmark}     &   Jun 2018        & Github \\
%     \texttt{TSB UAD, 2022}~\cite{paparrizos2022tsb-uad}         &   Nov 2022        & Github \\
%     \texttt{TODS, 2021}~\cite{lai2021todsbenchmark}             &   Jan 2021        & Paper \\
%     \texttt{TimeEval, 2022}~\cite{wenig2022timeeval}            &   Aug 2022        & Paper \\
%     \texttt{Exathlon, 2021}~\cite{jacob2020exathlon}            &   Sep 2021        & Paper \\
%     \texttt{Merlion, 2021}~\cite{bhatnagar2021merlion}          &   Sep 2021        & Paper \\
%     % \midrule
%     % \bench                                                      &   May 2023        & Github \\
%     \bottomrule
% \end{tabular}}

==> tables/benchmark_f1.tex <==
\begin{adjustbox}{angle=90}
\begin{table*}[!t]
\caption{Benchmark Summary Results}
\label{tab:bench_f1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccc}
\toprule
& \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo S5} & \multicolumn{5}{c}{NAB}  \\
\cmidrule(r){2-3}\cmidrule(r){4-7}\cmidrule(r){8-12}
\textbf{Pipeline} & MSL & SMAP & A1 & A2 & A3 & A4 & Art & AWS & AdEx & Traf & Tweets\\
\midrule
AER      &  0.616$\pm$0.02 &  0.788$\pm$0.01 &  0.778$\pm$0.01 &   0.982$\pm$0.00 &  0.885$\pm$0.01 &  0.711$\pm$0.01 &  0.736$\pm$0.12 &  0.732$\pm$0.02 &  0.708$\pm$0.04 &  0.688$\pm$0.03 &  0.571$\pm$0.02 \\
LSTM DT  &  0.485$\pm$0.01 &  0.709$\pm$0.02 &  0.732$\pm$0.02 &  0.977$\pm$0.01 &   0.740$\pm$0.01 &  0.649$\pm$0.01 &  0.404$\pm$0.03 &  0.491$\pm$0.03 &  0.743$\pm$0.01 &  0.638$\pm$0.04 &  0.556$\pm$0.01 \\
ARIMA    &   0.435$\pm$0.00 &   0.324$\pm$0.00 &   0.744$\pm$0.00 &   0.816$\pm$0.00 &   0.782$\pm$0.00 &   0.684$\pm$0.00 &   0.429$\pm$0.00 &   0.472$\pm$0.00 &   0.727$\pm$0.00 &   0.429$\pm$0.00 &   0.513$\pm$0.00 \\
LSTM AE  &  0.489$\pm$0.05 &  0.678$\pm$0.02 &  0.597$\pm$0.01 &  0.879$\pm$0.02 &  0.442$\pm$0.01 &  0.233$\pm$0.01 &  0.618$\pm$0.07 &  0.766$\pm$0.02 &  0.636$\pm$0.09 &   0.490$\pm$0.02 &  0.502$\pm$0.02 \\
TadGAN   &  0.558$\pm$0.05 &  0.598$\pm$0.02 &  0.577$\pm$0.03 &  0.818$\pm$0.01 &  0.402$\pm$0.02 &  0.343$\pm$0.02 &  0.567$\pm$0.06 &  0.627$\pm$0.03 &  0.678$\pm$0.09 &  0.532$\pm$0.04 &  0.528$\pm$0.04 \\
VAE      &  0.505$\pm$0.03 &  0.645$\pm$0.01 &  0.587$\pm$0.02 &  0.816$\pm$0.01 &  0.439$\pm$0.02 &  0.253$\pm$0.02 &  0.622$\pm$0.05 &   0.710$\pm$0.01 &  0.551$\pm$0.05 &  0.535$\pm$0.03 &  0.541$\pm$0.02 \\
Dense AE &  0.533$\pm$0.01 &  0.678$\pm$0.02 &  0.643$\pm$0.01 &  0.889$\pm$0.01 &  0.079$\pm$0.01 &  0.094$\pm$0.01 &   0.545$\pm$0.00 &  0.752$\pm$0.02 &  0.601$\pm$0.03 &  0.544$\pm$0.03 &   0.510$\pm$0.02 \\
GANF     &  0.438$\pm$0.02 &   0.463$\pm$0.00 &  0.095$\pm$0.01 &  0.156$\pm$0.01 &   0.008$\pm$0.00 &    0.150$\pm$0.00 &   0.667$\pm$0.00 &   0.578$\pm$0.00 &   0.308$\pm$0.00 &  0.556$\pm$0.02 &  0.673$\pm$0.01 \\
Azure AD &   0.051$\pm$0.00 &   0.019$\pm$0.00 &    0.280$\pm$0.00 &   0.653$\pm$0.00 &   0.702$\pm$0.00 &   0.344$\pm$0.00 &   0.054$\pm$0.00 &   0.112$\pm$0.00 &   0.244$\pm$0.00 &   0.111$\pm$0.00 &   0.189$\pm$0.00 \\
\bottomrule
\end{tabular}}
\end{table*}
\end{adjustbox}

==> tables/elapsed_time.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{l*{3}r}
    \toprule
                    & $<= 10,000$   & $> 10,000 <= 100,000$ & $> 100,000$ \\
    \midrule
    \texttt{AER}            & 0.46      &         2.16 (4.7$\times$)  &         11.00(5.1$\times$)  \\
    \texttt{LSTM DT}        & 0.33      &         1.38 (4.1$\times$)  &         6.49 (4.7$\times$)  \\
    \texttt{ARIMA}          & 0.45      &         5.79 (13$\times$)   &         7.61 (1.3$\times$)  \\
    \texttt{MP}             & 0.30      &         1.36 (4.6$\times$)  &         9.03 (6.7$\times$)  \\
    \texttt{LSTM AE}        & 0.25      &         1.22 (4.9$\times$)  &         7.29 (6$\times$)  \\
    \texttt{TadGAN}         & 1.48      &         5.44 (3.7$\times$)  &         32.97 (6.1$\times$) \\
    \texttt{VAE}            & 0.27      &         1.23 (4.5$\times$)  &         7.33 (6$\times$) \\
    \texttt{Dense AE}       & 0.06      &         0.39 (6.3$\times$)  &         2.82 (7.2$\times$) \\
    \texttt{GANF}           & 0.02      &         0.16 (7$\times$)    &         1.16 (7.5$\times$) \\
    \texttt{LNN}            & 3.83      &         21.47 (5.6$\times$) &         82.02 (3.8$\times$) \\
    \texttt{Azure AD}       & 0.03      &         0.04 (1.4$\times$)  &         0.03 (0.8$\times$) \\ 
    \texttt{AT}             & 0.20      &         1.59 (7.8$\times$)  &         10.70 (6.7$\times$) \\
    \bottomrule
    \end{tabular}
    \caption{Average runtime (minutes). TO BE DELETED}
    \label{tab:elapsed_time}
\end{table}


==> tables/version_change.tex <==
\begin{table}[t]
    \centering
    \caption{Percentage difference in average F1 score between releases and its standard deviation.}
    \begin{tabular}{lrl}
    \toprule
    {}                  &     \multicolumn{2}{l}{\% Change in F1 Score} \\
    \cmidrule(lr){2-3}
    Version Update      &   \multicolumn{1}{c}{$\mu$ $\pm$ $\delta$} & Explanation\\
    \midrule
    0.1.3 $\rightarrow$ 0.1.4 & \textbf{-3.92 $\pm$ 1.44} & E1: change in  metric calculation\\
    0.1.4 $\rightarrow$ 0.1.5 &  0.16 $\pm$ 0.25 \\
    0.1.5 $\rightarrow$ 0.1.6 & \textbf{1.11 $\pm$ 1.72} & E2: hyperparameter change\\
    0.1.6 $\rightarrow$ 0.1.7 &  0.30 $\pm$ 1.20 \\
    0.1.7 $\rightarrow$ 0.2.0 & -0.05 $\pm$ 0.82 \\
    0.2.0 $\rightarrow$ 0.2.1 & -0.52 $\pm$ 0.66 \\
    0.2.1 $\rightarrow$ 0.3.0 &  0.18 $\pm$ 1.16 \\
    0.3.0 $\rightarrow$ 0.3.1 &  0.25 $\pm$ 0.46 \\
    0.3.1 $\rightarrow$ 0.3.2 & -0.06 $\pm$ 0.79 \\
    0.3.2 $\rightarrow$ 0.4.0 & \textbf{0.16  $\pm$ 2.10} & E3: \texttt{TensorFlow} upgrade\\
    0.4.0 $\rightarrow$ 0.4.1 & -0.20 $\pm$ 0.62 \\
    0.4.1 $\rightarrow$ 0.5.0 &  0.08 $\pm$ 0.48 \\
    0.5.0 $\rightarrow$ 0.5.1 & \textbf{-2.60 $\pm$ 1.16} & E4: new dataset added\\
    0.5.1 $\rightarrow$ 0.5.2 & -0.10 $\pm$ 1.27 \\
    0.5.2 $\rightarrow$ 0.6.0 &  0.40 $\pm$ 0.86 \\
    \bottomrule
    \end{tabular}
    \label{tab:change}
\end{table}

==> textfiles/1.introduction_old.tex <==
\section{Introduction}

% widespread of time series anomaly detection models
As continuous data collection becomes more common place across domains, there is a corresponding need to monitor systems, devices, and even human health and activity in order to find patterns in collected data, as well as deviations from those patterns~\cite{chandola2009survey, aggarwal2017outlieranalysis}. Over the past decade, tremendous progress has been made in using machine learning to perform various types of monitoring, including unsupervised time series anomaly detection. 
For example, in the past 5 years, \citet{hundman2018lstmdt} created a forecasting Long Short-Term Memory (LSTM) model to find anomalies in spacecraft data, \citet{park2018vae} used LSTM variational autoencoders for anomaly detection in multimodal sensor signals collected from robotic arms, and \citet{geiger2020tadgan} used generative adversarial networks for time series anomaly detection on widely used public datasets.

% does it address user needs?

%When \textit{end-users} -- who we specifically define as people who are interested in training a model on their own data in order to find anomalies -- attempt to use these models, they regularly run into a few questions and challenges. 
%First, they often want to know: \textit{``am I using the state-of-the-art (SOTA) model, and how do I know that?"} 
%Second, with rapid innovations in the ML space and new modeling approaches frequently announced and publicized, \textit{"how can I keep up?"} 
%Third, if a model is said to be SOTA, \textit{``how can I trust that it is, before investing a lot of effort in using it for my data?"}
%The unsupervised nature of the problem accentuates this need, because unlike with predictive modeling, in unsupervised learning there is no ground truth, and it is always possible to monitor one's systems better. 
%Ultimately, it is important to note that an \user{} is only interested in finding the best solution for their particular problem, and does not think about these modeling techniques the same way researchers do. 

%KV version 

When \textit{end-users} -- who we specifically define as people who are interested in training a model on their own data in order to find anomalies -- attempt to use these models, they regularly run into a few questions and challenges. We highlight these here. 

\noindent \textbf{End-users' fear of missing out on state-of-the-art models.} First, end-users often want to know: \textit{``am I using the state-of-the-art (SOTA) model, and how do I know that?"} The unsupervised nature of the problem accentuates this need, because unlike with predictive modeling, in unsupervised learning there is no ground truth, and there is always the issue of ``unknown-unkowns", that is, a user may wonder if the new approach can reveal anomalies that were previously unseen. With rapid innovations in the ML space and new modeling approaches frequently announced and publicized, users find themselves in a constant phase of \textit{"how can I keep up?"} 

% Incorperation of the latest and greatest
\noindent \textbf{End-users' struggle of incorporating the latest state-of-the-art.} If ultimately the user decides to use a latest innovative pipeline, perhaps alongside their existing approach, one question is \textit{``how do I get started as research papers are full of new terminology published alongside obfuscated code?"}
 
Ultimately, it is important to note that an \user{} is only interested in finding the best solution for their particular problem, and does not think about these modeling techniques the same way researchers do. 


In recent years, benchmarks have become instrumental in gauging and comparing model performance for machine learning researchers ~\cite{coleman2019dawnbench, han2022adbench}. In this paper, we ask — can benchmarking frameworks also help to alleviate \user{s} challenges? While many time series anomaly detection benchmarks have been introduced~\cite{jacob2020exathlon, lai2021todsbenchmark, paparrizos2022tsb-uad, lavin2015numentabenchmark, wenig2022timeeval}, they are not directed toward \user{s}, and are usually not kept up-to-date. Table~\ref{tab:related_work} shows the latest published results for each time series anomaly detection benchmark framework, whether the score board has been updated on github, and the date of the latest update. Usually, these assessments are done once, during publication of related papers. Further comparisons are addressed in Section~\ref{sec:related}. We argue that this makes them \textit{point-in-time} benchmarking frameworks.  

% \begin{table}[t]
%     \centering
%     \caption{The latest published performance results for each benchmarking framework. These frameworks are \textit{point-in-time} benchmarks, lacking continuous updates.}
%     \input{tables/bench_frameworks}
%     \label{tab:frameworks}
% \end{table}

Still, we propose that with a few careful innovations, these benchmarking frameworks can further help \user{s}. With that in mind, in this paper, we propose \bench -- a user-centric benchmarking framework for unsupervised time series anomaly detection. Three concrete innovations enable us to address \user{s’} common but critical concerns: 
\begin{itemize}
\itemsep0em
\item A continuously running system, moving away from \textit{point-in-time} evaluations;  
\item Abstractions that allow us to easily incorporate and assess new models, and isolate the factors that make them better.
\item Seamless integration of the latest models into usable \textit{pipelines} for end-users. 
\end{itemize}

%Note for Sarah: I highlighted the most important, to least important, considering user centric. The end to end framework aspect, is arguable, because others have it too... 

\input{tables/related_work}

\indent\textbf{Why unsupervised learning?}
Anomalous events are rare and often difficult to recognize. End-users who search for them are often unable to determine \textit{what} they are looking for and \textit{when} anomalies occur in their data without an in-depth investigation. Supervised and unsupervised machine learning models can help end-users search for anomalous events. With supervised learning, models learn patterns from human-labelled data and then use them to detect other anomalies. Because these models are restricted to previously labelled events that are themselves difficult for humans to find, it can be difficult for such models to make useful predictions with limited labelled data. Moreover, these models struggle to find ``new'' events that are interesting to the end-user. In contrast, unsupervised learning models do not rely on labels, and flag any intervals that deviate from the expected pattern, possibly addressing the aforementioned challenge of ``unknown-unkowns" where end-users search for events that were previously undiscovered. 
\textit{OrionBench} focuses on \underline{unsupervised} models.

Below we highlight our framework's unique contributions. \bench is: 
\begin{enumerate}
    \item \textbf{An extensible framework} that enables the integration of new pipelines and datasets. \bench started with 2 pipelines in 2020, and as of now encompasses 12 pipelines, 27 primitives, 14 public datasets, and 2 custom evaluation metrics. Once integrated into the framework and benchmarked, the pipeline is seamlessly made available to the \user{} through unified APIs.
    \item \textbf{A continuously-run benchmark} with frequent releases. To date, we have 14 benchmark leaderboards over the course of almost three years, starting in September 2020. Our latest release in October 2023 makes for an overall accumulation of 52,966 experiments. We demonstrate the stability and reproducibility of \bench by showcasing the progression of pipeline performances across all releases to date.
    \item \textbf{Open-source} and publicly available \url{https://github.com/sintel-dev/Orion} under an MIT license.
    \item  \textbf{An end-to-end benchmark} executable with a single command. Given a pipeline and datasets, the benchmark evaluates the performance of the pipeline on every signal according to time series anomaly detection-based metrics. We provide an extensive evaluation that illustrates the qualitative and computational performances of pipelines across all datasets.
\end{enumerate}

% section description
The remainder of the paper is organized as follows:
In Section~\ref{sec:related}, we compare \bench to existing open-source benchmarking frameworks. We detail the user-centric components of \bench in Section~\ref{sec:system}. Section~\ref{sec:demo} presents an evaluation of our benchmarking framework and describes two real scenarios in which \bench was valuable. We conclude in Section~\ref{sec:discussion}.

